First measurement of the ratio of $\psi(2S)$-to-$J/\psi$ inclusive production in $p\mathrm{Ar}$ and $pp$ collisions at $\sqrt{s_{\mathrm{NN}}} =113\,\mathrm{GeV}$ with SMOG2

A measurement of the $\psi(2S)$-to-$J/\psi$ production cross-section ratio is performed in proton-argon ($p\mathrm{Ar}$) and proton-proton ($pp$) collisions in fixed-target mode at $\sqrt{s_{\mathrm{NN}}}=113\,\mathrm{GeV}$. Data samples were collected by the LHCb experiment during argon and hydrogen gas injections in the SMOG2 storage cell, resulting in $p\mathrm{Ar}$ and $pp$ collisions, respectively. The $\psi(2S)$-to-$J/\psi$ production cross-section ratio is measured as a function of the charmonium transverse momentum, $p_{\mathrm{T}}$, and rapidity in the centre-of-mass system, $y^{*}$. The $\psi(2S)$-to-$J/\psi$ ratio in $p\mathrm{Ar}$ collisions over that in $pp$ collisions is measured to be $0.90 \pm 0.04 \pm 0.02$ for $-2.3<y^{*}<0.0$ and $0<p_{\mathrm{T}}<8\mathrm{GeV}/c$, indicating the emergence of nuclear effects in the $p\mathrm{Ar}$ system. This study acts as a baseline for the interpretation of future measurements with larger systems accessible by the LHCb experiment.

==> Authorship_LHCb-PAPER-2026-026-arXiv.tex <==
LHCb collaboration:
R. Aaij,
M. Abdelfatah,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin\'en,
T. Ackernley,
A.A. Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
S. Akar,
K. Akiba,
H. Al Saleh,
P. Albicocco,
J. Albrecht,
R. Aleksiejunas,
F. Alessio,
P. Alvarez Cartelle,
S. Amato,
J.L. Amey,
Y. Amhis,
Z. Amos,
L. An,
L. Anderlini,
P. Andreola,
M. Andreotti,
S. Andres Estrada,
A. Anelli,
D. Ao,
C. Arata,
F. Archilli,
Z. Areg,
M. Argenton,
S. Arguedas Cuendis,
L. Arnone,
M. Artuso,
E. Aslanides,
R. Ata\'ide Da Silva,
M. Atzeni,
B. Audurier,
J.A. Authier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
M. Bai,
Z.B. Bai,
V. Balagura,
A. Balboni,
W. Baldini,
Z. Baldwin,
L. Balzani,
H. Bao,
J. Baptista de Souza Leite,
C. Barbero Pretel,
M. Barbetti,
I.R. Barbosa,
W. Barker,
R.J. Barlow,
M. Barnyakov,
S. Baron,
S. Barsuk,
W. Barter,
J. Bartz,
S. Bashir,
B. Batsukh,
P.B. Battista,
A. Bavarchee,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
N.A. Behling,
S. Belin,
A. Bellavista,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
J.L.M. Berkey,
R. Bernet,
A. Bertolin,
L. Bertsch,
F. Betti,
J. Bex,
O. Bezshyyko,
S. Bhattacharya,
M.S. Bieker,
N.V. Biesuz,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Bohare,
C. Bolognani,
R.B. Bonacci,
A. Bordelius,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
E. Bottalico,
S.A. Bouchiba,
M. Bovill,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
J.D. Brandenburg,
A. Brea Rodriguez,
N. Breer,
C. Breitfeld,
J. Brodzicka,
J. Brown,
E. Buchanan,
M. Burgos Marcos,
C. Burr,
E. Butera,
C. Buti,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
Y. Cai,
Y. Cai,
A. Caillet,
R. Calabrese,
L. Calefice,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J.I. Cambon Bouzas,
P. Campana,
A. Campomagnani,
A.C. Campos,
A.F. Campoverde Quezada,
Y. Cao,
S. Capelli,
M. Caporale,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
R. Caspary,
G. Casse,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
I. Celestino,
S. Cesare,
A.J. Chadwick,
M. Charles,
Ph. Charpentier,
E. Chatzianagnostou,
R. Cheaib,
M. Chefdeville,
C. Chen,
J. Chen,
S. Chen,
Z. Chen,
A. Chen Hu,
M. Cherif,
S. Chernyshenko,
X. Chiotopoulos,
G. Chizhik,
V. Chobanova,
A. Christakakis,
M. Chrzaszcz,
Y. Chu,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
A. Codovini,
C. Codovini,
J. Cogan,
E. Cogneras,
L. Cojocariu,
S. Collaviti,
P. Collins,
T. Colombo,
M. Colonna,
A. Comerma-Montells,
L. Congedo,
J. Connaughton,
A. Contu,
N. Cooke,
A. Corallo,
G. Cordova,
C. Coronel,
I. Corredoira ,
A. Correia,
G. Corti,
G.C. Costantino,
C. Cotirlan,
J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
N. Crepet,
M. Cruz Torres,
M. Cubero Campos,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
X. Dai,
J. Dalseno,
C. D'Ambrosio,
G. Darze,
A. Davidson,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
F. De Gregorio,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
A. De Robertis,
E. De Santis,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
S. Dekkers,
L. Del Buono,
B. Delaney,
B. Demaire-Lepape,
J. Deng,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
S. Ding,
Y. Ding,
L. Dittmann,
J.F. Diverchy,
A.D. Docheva,
A. Doheny,
C. Dong,
F. Dordei,
J. Dorta Moreno,
A.C. dos Reis,
J. Dos Santos Oliveira,
A.D. Dowling,
L. Dreyfus,
W. Duan,
P. Duda,
L. Dufour,
V. Duk,
P. Durante,
M.M. Duras,
J.M. Durham,
O.D. Durmus,
K. Duwe,
A. Dziurda,
S. Easo,
E. Eckstein,
U. Egede,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
D. Elizondo Blanco,
J. Ellbracht,
S. Ely,
A. Ene,
T. Evans,
F. Fabiano,
S. Faghih,
L.N. Falcao,
B. Fang,
R. Fantechi,
L. Fantini,
M. Faria,
K. Farmer,
F. Fassin,
D. Fazzini,
L. Felkowski,
C. Feng,
M. Feng,
A. Fernandez Casani,
M. Fernandez Gomez,
B. Fernandez Rodino,
J. Fernandez-John,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
R.A. Fini,
R. Fiorenza,
M. Fiorini,
M. Firlej,
D.S. Fitzgerald,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
A. Fomin,
M. Fontana,
M. Fontes Vaz,
L.A. Foreman,
R. Forty,
D. Foulds-Holt,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Y. Fu,
Q. F\"uhring,
T. Fulghesu,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B. Ganie,
H. Gao,
R. Gao,
T.Q. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc\'ia Pardi\~nas,
P. Gardner,
L. Garrido,
C. Gaspar,
A. Gavrikov,
J. George,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
S. Ghizzo,
Z. Ghorbanimoghaddam,
F.I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent\`u,
L. Girardey,
M.A. Giza,
F.C. Glaser,
V.V. Gligorov,
C. G\"obel,
L. Golinka-Bezshyyko,
E. Golobardes,
A. Golutvin,
S. Gomez Fernandez,
A.G. Gomez Mongui,
W. Gomulka,
F. Goncalves Abrantes,
I. Gon\c{c}ales Vaz,
M. Goncerz,
G. Gong,
S. Gong,
J.A. Gooding,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
L.A. Granado Cardoso,
R. Grande Quartieri,
E. Graug\'es,
E. Graverini,
L. Grazette,
G. Graziani,
A.T. Grecu,
N.A. Grieser,
L. Grillo,
C. Gu,
M. Guarise,
L. Guerry,
A.-K. Guseinov,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S. Haken,
G. Hallett,
P.M. Hamilton,
Q. Han,
S. Han,
X. Han,
S. Hansmann-Menzemer,
N. Harnew,
T.J. Harris,
L. Hartman,
M. Hartmann,
S. Hashmi,
M. Haubner,
J. He,
N. Heatley,
A. Hedes,
F. Hemmer,
C. Henderson,
R. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
A. Henrot,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Heyn,
A. Hicheur,
G. Hijano Mendizabal,
J. Horswill,
R. Hou,
Y. Hou,
D.C. Houston,
N. Howarth,
W. Hu,
X. Hu,
W. Hulsbergen,
R.J. Hunter,
D. Hutchcroft,
M. Idzik,
P. Ilten,
A. Iohner,
S. Jacevicius,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
T. Jakoubek,
E. Jans,
A. Jawahery,
C. Jayaweera,
A. Jelavic,
V. Jevtic,
Z. Jia,
E. Jiang,
X. Jiang,
Y. Jiang,
Y.J. Jiang,
E. Jimenez Moya,
N. Jindal,
M. John,
A. John Rubesh Rajan,
D. Johnson,
C.R. Jones,
S. Joshi,
B. Jost,
J. Juan Castella,
N. Jurik,
I. Juszczak,
K. Kalecinska,
D. Kaminaris,
S. Kandybei,
M. Kane,
Y. Kang,
C. Kar,
M. Karacson,
A. Kauniskangas,
J.W. Kautz,
M.K. Kazanecki,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
S. Kholodenko,
V. Kholoimov,
G. Khreich,
F. Kiraz,
T. Kirn,
V.S. Kirsebom,
N. Kleijne,
A. Kleimenova,
D. Klekots,
K. Klimaszewski,
M.R. Kmiec,
T. Knospe,
R. Kolb,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
A. Korchin,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
E. Kowalczyk,
O. Kravcov,
M. Kreps,
W. Krupa,
W. Krzemien,
O. Kshyvanskyi,
S. Kubis,
M. Kucharczyk,
A. Kupsc,
A. Kurzina,
V. Kushnir,
B. Kutsenko,
J. Kvapil,
I. Kyryllin,
D. Lacarrere,
P. Laguarta Gonzalez,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
H. Lee,
R. Lef\`evre,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
E.D. Lesser,
B. Leverington,
A. Li,
C. Li,
C. Li,
H. Li,
J. Li,
K. Li,
L. Li,
L. Li,
P. Li,
P.-R. Li,
Q. Li,
T. Li,
T. Li,
W. Li,
Y. Li,
Y. Li,
Y. Li,
Z. Li,
Z. Lian,
Q. Liang,
X. Liang,
Z. Liang,
S. Libralon,
A. Lightbody,
J. Lin,
S. Lin,
T. Lin,
R. Lindner,
H. Linton,
R. Litvinov,
D. Liu,
F.L. Liu,
G. Liu,
K. Liu,
S. Liu,
W. Liu,
X. Liu,
Y. Liu,
Y. Liu,
Y.L. Liu,
G. Loachamin Ordonez,
I. Lobo,
A. Lobo Salvia,
A. Loi,
T. Long,
F.C.L. Lopes,
J.H. Lopes,
A. Lopez Huertas,
C. Lopez Iribarnegaray,
Q. Lu,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
Y. Luo,
A. Lupato,
M. Lupberger,
E. Luppi,
K. Lynch,
J. Lyu,
S. Lyu,
X.-R. Lyu,
H. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B. Mack,
I. Mackay,
L.M. Mackey,
L.R. Madhan Mohan,
M.J. Madurai,
D. Magdalinski,
J.J. Malczewski,
S. Malde,
L. Malentacca,
G. Manca,
C. Mancuso,
R. Manera Escalero,
A. Mangalasseri,
F.M. Manganella,
R. Mangrulkar,
D. Manuzzi,
S. Mao,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
L. Mareso,
E. Mariani,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
L. Martel,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
C. Martinez,
A. Martinez Armas,
D. Martinez Gomez,
D. Martinez Santos,
F. Martinez Vidal,
A. Martorell i Granollers,
A. Massafferri,
R. Matev,
A. Mathad,
C. Matteuzzi,
K.R. Mattioli,
L. Matzner,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
J. Mazorra de Cos,
M. Mazurek,
D. Mazzanti Tarancon,
M. McCann,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
S.E.R. Medaer,
D. Melnychuk,
D. Mendoza Granada,
P. Menendez Valdes Perez,
F.M. Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
S. Mico,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
B. Mitreska,
D.S. Mitzel,
R. Mocanu,
A. Modak,
L. Moeser,
R.D. Moise,
E.F. Molina Cardenas,
T. Momb\"acher,
M. Monk,
T. Monnard,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A. Moro,
J. Moron,
W. Morren,
A.B. Morris,
A.G. Morris,
R. Mountain,
Z. Mu,
N. Muangkod,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M\"uller,
F. Mu\~noz-Rojas,
V. Mytrochenko,
P. Naik,
T. Nakada,
R. Nandakumar,
G. Napoletano,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
J. Nicolini,
D. Nicotra,
E.M. Niel,
L. Nisi,
Q. Niu,
B.K. Njoki,
P. Nogarolli,
P. Nogga,
J. Nombela Royo,
C. Normand,
A. Novo Cal,
J. Novoa Fernandez,
G. Nowak,
H.N. Nur,
A. Oblakowska-Mucha,
T. Oeser,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
E. Olivart Pino,
M. Olocco,
R.H. O'Neil,
J.S. Ordonez Soto,
D. Osthues,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
F. Paciolla,
A. Padee,
K.O. Padeken,
B. Pagare,
T. Pajero,
A. Palano,
L. Palini,
L. Palombini,
M. Palutan,
C. Pan,
X. Pan,
S. Panebianco,
S. Paniskaki,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
D. Parmar,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A. Paul,
C.J. Pawley,
A. Pellegrino,
J. Peng,
X. Peng,
M. Pepe Altarelli,
S. Perazzini,
H. Pereira Da Costa,
M. Pereira Martinez,
A. Pereiro Castro,
C. Perez,
A. Perez Casas,
P. Perret,
A. Perrevoort,
A. Perro,
M.J. Peters,
A. Petkovic,
K. Petridis,
A. Petrolini,
S. Pezzulo,
J.P. Pfaller,
H. Pham,
L. Pica,
M. Piccini,
L. Piccolo,
B. Pietrzyk,
R.N. Pilato,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V.M. Placinta,
M. Plo Casasus,
T. Poeschl,
F. Polci,
M. Poli Lener,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
S. Ponce,
D. Popov,
K. Popp,
K. Prasanth,
C. Prouve,
D. Provenzano,
V. Pugatch,
A. Puicercus Gomez,
G. Punzi,
J.R. Pybus,
Q. Qian,
W. Qian,
N. Qin,
R. Quagliani,
R.I. Rabadan Trejo,
B. Rachwal,
R. Racz,
J.H. Rademacker,
M. Rama,
M. Ram\'irez Garc\'ia,
V. Ramos De Oliveira,
M. Ramos Pernas,
G. Ramsey,
M.S. Rangel,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
M. Ribalda Galvez,
R. Ribatti,
G. Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
F. Riehn,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
A. Rodriguez Alvarez,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
J. Roensch,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
A. Romano,
V. Romanovskiy,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
W. Rose,
M. Rotondo,
M.S. Rudolph,
G. Ruggiero,
M. Ruiz Diaz,
J. Ruiz Vidal,
J. Ruz Armendariz,
J.J. Saavedra-Arias,
J.J. Saborido Silva,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
A. Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
H. Sazak,
F. Sborzacchi,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
N. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
H. Schumacher,
M.H. Schune,
G. Schwering,
B. Sciascia,
A. Sciuccati,
G. Scriven,
I. Segal,
S. Sellam,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
B. Sevilla Sanjuan,
Y. Shang,
D.M. Shangase,
R.S. Sharma,
L. Shchutska,
T. Shears,
S. Shelton,
J. Shen,
Z. Shen,
S. Sheng,
B. Shi,
J. Shi,
Q. Shi,
W.S. Shi,
E. Shmanin,
R. Silva Coutinho,
G. Simi,
S. Simone,
M. Singha,
I. Siral,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
E. Smith,
M. Smith,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
K. Solovieva,
N.S. Sommerfeld,
R. Song,
Y. Song,
Y. Song,
Y.S. Song,
F.L. Souza De Almeida,
G. Souza De Castro,
B. Souza De Paula,
K.M. Sowa,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
M. Stefaniak,
O. Steinkamp,
F. Suljik,
J. Sun,
L. Sun,
M. Sun,
D. Sundfeld,
P. Svihra,
V. Svintozelskyi,
J. Swallow,
K. Swientek,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
Y. Tang,
Y.T. Tang,
M.D. Tat,
J.A. Teijeiro Jimenez,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
A.R. Thomson-Strong,
R. Thornton,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
T.T. Todorov,
L. Tomassetti,
G. Tonani,
X. Tong,
T. Tork,
L. Torlai,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
A. Upadhyay,
B. Urbach,
A. Usachov,
U. Uwer,
V. Vagnoni,
A. Vaitkevicius,
A. Valassi,
V. Valcarce Cadenas,
G. Valenti,
N. Valls Canudas,
J. van Eldik,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
P. Varrella,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V\'azquez Sierra,
S. Vecchi,
J. Velilla Serna,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Verdoglia,
M. Vesterinen,
W. Vetens,
D. Vico Benet,
P. Vidrier Villalba,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
B. Vivacqua,
F.C. Volle,
D. vom Bruch,
K. Vos,
C. Vrahas,
J. Wagner,
J. Walsh,
N. Walter,
E.J. Walton,
G. Wan,
A. Wang,
B. Wang,
C. Wang,
C. Wang,
C. Wang,
G. Wang,
H. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N.W. Wang,
X. Wang,
X. Wang,
X. Wang,
X.W. Wang,
Y. Wang,
Y. Wang,
Y. Wang,
Y.H. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
A. Wasili,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
Z. Weida,
J. Wendel,
B.D.C. Westhenry,
A.S. White,
C. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
M.A. Wiegertjes,
C. Wild,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.J. Williams,
M.R.J. Williams,
R. Williams,
S. Williams,
Z. Williams,
F.F. Wilson,
M. Winn,
W. Wislicki,
M. Witek,
L. Witola,
T. Wolf,
E. Wood,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
T. Wu,
X. Wu,
Y. Wu,
Z. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
T.X. Xing,
A. Xu,
L. Xu,
M. Xu,
R. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
S. Yadav,
K. Yang,
X. Yang,
Y. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
H. Yeung,
H. Yin,
X. Yin,
C.Y. Yu,
J. Yu,
K. Yu,
X. Yuan,
Y Yuan,
S. Zalambani,
J.A. Zamora Saa,
F. Zangari,
M. Zavertyaev,
M. Zdybal,
F. Zenesini,
C. Zeng,
M. Zeng,
S.H Zeng,
C. Zhang,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
Q.Z. Zhang,
R. Zhang,
S. Zhang,
S.L. Zhang,
Y. Zhang,
Z. Zhang,
J. Zhao,
M. Zhao,
Y. Zhao,
A. Zhelezov,
S.Z. Zheng,
X.Z. Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
V. Zhovkovska,
L.Z. Zhu,
X. Zhu,
X. Zhu,
Y. Zhu,
V. Zhukov,
J. Zhuo,
T. Zies,
D. Zuliani,
X. Zuo
